Learning Reward Functions from Diverse Sources of Human Feedback: Optimally Integrating Demonstrations and Preferences

Reward functions are a common way to specify the objective of a robot. As designing reward functions can be extremely challenging, a more promising approach is to directly learn reward functions from human teachers. Importantly, data from human teachers can be collected either passively or actively in a variety of forms: passive data sources include demonstrations, (e.g., kinesthetic guidance), whereas preferences (e.g., comparative rankings) are actively elicited. Prior research has independently applied reward learning to these different data sources. However, there exist many domains where multiple sources are complementary and expressive. Motivated by this general problem, we present a framework to integrate multiple sources of information, which are either passively or actively collected from human users. In particular, we present an algorithm that first utilizes user demonstrations to initialize a belief about the reward function, and then actively probes the user with preference queries to zero-in on their true reward. This algorithm not only enables us combine multiple data sources, but it also informs the robot when it should leverage each type of information. Further, our approach accounts for the human's ability to provide data: yielding user-friendly preference queries which are also theoretically optimal. Our extensive simulated experiments and user studies on a Fetch mobile manipulator demonstrate the superiority and the usability of our integrated framework.

==> notes.tex <==
\section{Problem Formulation}

\newcommand{\states}{\mathcal{S}}
\newcommand{\actions}{\mathcal{A}}

\textbf{Model.} We consider a deterministic, fully-observable dynamical system. At time $t$, $s_t\in \states$ denotes the state of the system and $a_t\in\actions$ denotes the control input (action) to the system. A trajectory, $\xi\in\Xi$, is a sequence of state-action pairs, i.e., $\xi = ((s_t, a_t))_{t=0}^T$, where $T$ is the finite time horizon of the system. Because the system is deterministic, a trajectory $\xi$ can be more succinctly represented by $\Lambda = (s_0, a_0, a_1, \ldots, a_T)$, the initial state and sequence of actions in the trajectory. We use $\xi$ and $\Lambda$ interchangeably when referring to a trajectory, depending on the context.

We assume how a human wants the system to behave is described by a reward function, $R: \Xi \to \mathbb{R}$. Our goal is to learn $R$. More formally, let $R$ be a linear combination of some trajectory features $\Phi: \Xi \to \mathbb{R}^d$, so that $R(\xi) = \omega^\top \Phi(\xi)$ for some $\norm{\omega}_2\leq 1$. To learn $R$, we must simply learn the human's $\omega$.


\textbf{Demonstrations.} A \emph{demonstration} data set is a set of trajectories $\mathcal{D}:=\{\xi^D_1, \xi^D_2,\mydots,\xi^D_L\}$ demonstrated by the human. These trajectories align with the human's preferences. We will use this data set to learn an initial posterior distribution over the reward parameter $\omega$. By assuming a noisily optimal human demonstration model
\begin{align}
    P(\xi^D_l \mid \omega) \propto \exp{\left(\beta^DR(\xi^D_l)\right)} = \exp{\left(\beta^D\omega^\top\Phi(\xi^D_l)\right)}
\end{align}
where $\beta^D\geq0$ is a temperature parameter that models how noisy the human demonstrations are, we will use BIRL \citep{ramachandran2007bayesian} to obtain this posterior distribution:
\begin{align}
    P(\omega \mid \mathcal{D}) &\propto P(\omega)P(\mathcal{D} \mid \omega) \nonumber\\
    &= P(\omega)\prod_{l=1}^{L} P(\xi^D_l \mid \omega) \;.
\end{align}
where the equality formalizes the conditional independence between the demonstrations. Assuming a uniform prior distribution $P(\omega)$ over the unit ball $\{\omega \mid \norm{\omega}_2\leq 1\}$, we write
\begin{align}
    P(\omega \mid \mathcal{D}) \propto \prod_{l=1}^{L} \exp{\left(\beta^D\omega^\top\Phi(\xi^D_l)\right)}
\end{align}
for any $\omega$ in the unit ball. We will then use this initial posterior to better learn $\omega$ via preference queries.


\textbf{Preference Queries.} A \emph{preference query} $Q:=\{\xi_1,\xi_2,\mydots,\xi_K\}$ is a set of $K$ trajectories; the human responds to a preference query by picking the trajectory they most prefer from this set. After performing BIRL to learn an initial posterior, we will regard it as our prior and update this distribution by choosing---and having the human respond to---a sequence of queries.

We want to find the true reward parameter using as few preference queries as tractably possible. In other words, we want to find the sequence of queries that maximizes the amount of information we expect to receive about $\omega$. Such a sequence of queries should recognize there is a human-in-the-loop, and so should generate queries that are ``easy" for the human, thereby minimizing the amount of bad feedback it may receive. Unfortunately, this problem is NP-hard \citep{ailon2012active}.

Therefore, we proceed in a greedy fashion: after initializing the prior distribution over $\omega$ using the demonstration data set $\mathcal{D}$, we iteratively alternate between (a) generating a single query and (b) using the human's response to that query to update our distribution. In this paper, we present two different query generation strategies: the maximum volume removal method \citep{sadigh2017active} and the maximum information gain method \citep{biyik2019asking}, both of which have bounded regret.

We first focus on the second step: updating our prior distribution over $\omega$ based on the human's response. Let $P(q \mid Q, \omega)$ denote the probability that the human chooses trajectory $q$ from the query $Q$ when their reward parameter is $\omega$ (see Section~\ref{sec:human_model} for common human choice models). Then, given the prior $p(\omega \mid \mathcal{D})$ and the human's response $q$ to the query $Q$, we can compute a posterior over $\omega$:
\begin{align}
P(\omega \mid Q,q,\mathcal{D}) &\propto P(q \mid Q,\omega,\mathcal{D})P(\omega \mid \mathcal{D}) \nonumber\\
&= P(q \mid Q,\omega)P(\omega \mid \mathcal{D})
\end{align}
where the equality is because the human's response to a query is solely determined by $\omega$, and so conditionally independent from the demonstration data set $\mathcal{D}$. In the next sections, we discuss methods for generating the queries $Q$ that the human will answer.















% Iterated Correction and Batch-mode Active Methods 
Finally, we now discuss the extensions for the active preference-based learning stage which further accelerates the learning or enhances its practicality.

\noindent \textbf{Iterated Correction.} \cite{palan2019learning} proposed a heuristic method to guide the volume removal optimization towards another local optima that can ease the job of the human in responding to the queries. In this extension, each and every query is appended with a trajectory that is known to be preferred by the human. To do that, the first preference-query is appended with a demonstration, and the later queries are appended with the trajectory that the human selected in the previous query. Formally, denoting this trajectory-to-be-appended with $\Lambda^A$, the optimization problem becomes
\begin{align}
Q^*_i \asymeq &\argmin_{Q_i=\{\Lambda_1,\dots,\Lambda_K\}}\sum_{q_i\in Q_i}\left(\sum_{{\omega}\in\Omega}P(q_i\mid Q_i,{\omega})\right)^2\nonumber\\
&\quad\textrm{subject to}\quad \Lambda^K = \Lambda^A
\label{eq:final_old_optimization}
\end{align}

While, technically, the information gain method can also be extended with this iterated correction heuristic, it is not necessary because the method inherently generates easy questions. Therefore, iterated correction can be thought as an attempt specifically for the volume removal method to generate easier questions similar to the information gain method. 

\noindent \textbf{Batch-mode Active Methods.} \cite{biyik2018batch} and \cite{biyik2019batch} proposed batch-mode active preference query generation methods that output a batch of queries instead of greedily selecting one query at a time. These methods attempt to balance a good trade-off between queries' informativeness and diversity to avoid redundancy within batches. While both works used the volume removal objective value for each query as the metric for informativeness, the same techniques readily apply with the information gain objective value.


\section{Volume Removal}

Theorem~\ref{thm:volume_removal_failure} and Example~\ref{ex:example_question} demonstrate the maximum volume removal method works well in practice not despite the non-convexity of the optimization problem, but thanks to it. This non-convexity allows solution methods to converge to other locally optimal queries, which may be easy for the human or more informative than the globally optimal trivial query.

We will call this method of learning from demonstrations and preference queries generated by volume removal \textsc{DemPref-VR} in short.

\noindent \textbf{Theoretical Guarantees.} \cite{sadigh2017active} have demonstrated, by virtue of the maximum volume removal objective being submodular, the greedy volume removal optimization is guaranteed to have bounded sub-optimality in terms of the volume removed under some assumptions. Considering \textsc{DemPref-VR} as an identical method except the prior that is now learned via human demonstrations, \textsc{DemPref-VR} also has the same theoretical guarantees, because the preference-based learning stage is unaffected.

The optimal stopping condition is valid only for the information gain and adapting it to the volume removal method is not trivial. This is because the volume removal objective includes an unnormalized probability distribution, which prevents us to bound the objective value, whereas the expected information gain is always upper bounded by the same quantity of the previous iteration. We use this property in the proof of Theorem~\ref{thm:optimal_stopping}.

All in all, when compared to the volume removal, the information gain method (1) has the same theoretical guarantees; (2) has the same computational complexity; (3) does not have a fundamental failure case; (4) generates easier queries for the human to respond; and (5) can leverage the same extensions.
